SASHIMI-SIDM: Semi-analytical subhalo modelling for self-interacting dark matter at sub-galactic scales

We combine the semi-analytical structure formation model, SASHIMI, which predicts subhalo populations in collisionless, cold dark matter (CDM), with a parametric model that maps CDM halos to self-interacting dark matter (SIDM) halos. The resulting model, SASHIMI-SIDM, generates SIDM subhalo populations down to sub-galactic mass scales, for an arbitrary input cross section, in minutes. We show that SASHIMI-SIDM agrees with SIDM subhalo populations from high-resolution cosmological zoom-in simulations in resolved regimes. Crucially, we predict that the fraction of core-collapsed subhalos peaks at a mass scale determined by the input SIDM cross section and decreases toward higher halo masses, consistent with the predictions of gravothermal models and cosmological simulations. For the first time, we also show that the core-collapsed fraction decreases toward lower halo masses. While the dependence of the collapse time on mass and concentration implies such behaviour, our semi-analytical approach allows us to quantify and illustrate this trend clearly across the full mass spectrum of subhalos, including for subhalo masses below the resolution limit of any current cosmological SIDM simulation. As a proof of principle, we apply SASHIMI-SIDM to predict the boost to the local dark matter density and annihilation rate from core-collapsed SIDM subhalos, which can be enhanced relative to CDM by an order of magnitude for viable SIDM models. Thus, SASHIMI-SIDM provides an efficient and reliable tool for scanning SIDM parameter space and testing it with astrophysical observations. The code is publicly available at https://github.com/shinichiroando/sashimi-si.

==> notes.tex <==
%Section 1

%Various observations at sub-galactic scales suggested problems for the cold dark matter (CDM) paradigm, which assumes that dark matter particles have a small velocity dispersion and do not interact with themselves or any standard-model particles.They include cusp-core, diversity, too-big-to-fail, and too-many-satellites problems~\cite{Bullock:2017xww}.Self-interacting dark matter (SIDM) has been introduced to solve some of these problems~\cite{Spergel:1999mh}, having attracted strong attention from multiple communities of particle physics, astrophysics and cosmology~\cite{Tulin:2017ara}.

%redistribuiting them in the phase space.If the density is sufficiently high and the scattering timescale is shorter than the age of the halo, this will %make a flat core towards the central region of the halo, which is in contrast to the $r^{-1}$ density cusp expected for CDM halos.The heat generated by %the self scattering will keep flowing from inner to outer region of the halo, which eventually induces the phenomenon called `gravothermal core collapse'.
%The time scale of the gravothermal core collapse depends on the halo properties (e.g., mass, density profile) as well as the SIDM scattering cross section per unit mass, $\sigma / m_\chi$.It was suggested that the core collapse was more efficient for dark matter subhalos as the steeper density slope due to the tidal effects at outskirts would make the core-collpase timescale shorter.

%This makes SIDM an attractive dark matter candidate, as it can explain diversity in the subhalos' density profiles.Some satellite galaxies are known to have cores, while the others have cusps, which can be explained by different evolution histories of SIDM subhalos that host each satellite galaxy.

%To tackle this by connecting with different parameterisation of the scattering cross section, the numerical simulations have been the leading tool.In this paper, we propose a semi-analytical model of SIDM as a complementary tool, which can address several shortcomings of the traditional approach based on the numerical simulations.Such an attempt was made espeically for, e.g., CDM, and we focus on one of the tools, \textbf{S}emi-\textbf{A}nalytical \textbf{S}ub\textbf{H}alo \textbf{I}nference \textbf{M}odell\textbf{I}ng, (SASHIMI).\footnote{\texttt{https://github.com/shinichiroando/sashimi-c}}

%Based on structure-formation theories, SASHIMI can compute subhalo populations efficiently, avoiding numerical resolution and shot noise inevitable for simulation-based approaches.
%Being in good agreement with outcomes of simulation simulations (mass functions~\cite{Hiroshima:2018kfv}, distribution of density profile parameters~\cite{Ando:2020yyk}), SASHIMI provides the most reliable way of extending the simulation results into sub-resolution regime, which can be probed with current and future generations of surveys such as the James Webb Space Telescope (JWST), Rubin Observatory Legacy Survey of Space and Time (LSST), and the Euclid satellite. 

%Combined with SASHIMI, we adopt a parameteric model of SIDM --- maping CDM subhalos to the corresponding SIDM subhalos --- obtained by comparing the CDM and SIDM cosmological simulations~\cite{Yang:2023jwn}.

%We demonstrate the good level of agreement of the SASHIMI-SIDM's predictions on the subhalo distributions of their density profile characteristics represented by quantities such as $V_{\rm max}$ and $r_{\rm max}$ (the maximum rotation speed and the radius at which the speed reaches this value, respectively).

% Section 2

%r_c^{\rm SIDM}(t) &=& r_{s}^{\rm CDM}(t_f)\left(2.555\tilde t^{1/2}-3.632\tilde t+2.131\tilde t^2-1.415\tilde t^3+0.4683\tilde t^4\right),

%The parameters for CDM can be related to one another through Eqs.~(\ref{eq:rho_s-V_max}) and (\ref{eq:r_s-r_max}).

%Considering the dimension of parameters, we can derive two scaling relations: $r_s(kr_{\rm max},kr_c)=kr_s(r_{\rm max},r_c)$ and $r_{\rm max}(r_s,r_c) = r_s x_{\rm max}(r_c/r_s)$, where $x_{\rm max}$ is the radius (normalized by $r_s$) at which the circular velocity is maximized:
%\begin{eqnarray}
%    x_{\rm max} &= & \mathrm{argmax}_{x=r/r_s} V_{\rm circ}, \\
%    V_\mathrm{circ}(r) &=& \left[\frac{4\pi G}{r}\int_0^r{{r'}^2\rho_\mathrm{SIDM}(r')}d{r'}\right]^{1/2}.
%\end{eqnarray}
%These relations allow us to calculate $r_s$ from ($r_{\rm max}$, $r_c$) as $r_s(r_{\rm max},r_c)=r_c/f_{\rm aux}(r_{\rm max}/r_c)$, where $f_{\rm aux}(k)$ is defined by $f_{\rm aux}(k) = x_c$ such that $kx_c=x_{\rm max}(x_c)$.

%Figures~\ref{fig:PDF_Vmax} and \ref{fig:PDF_rmax} show one-dimensional distribution functions of $V_{\rm max}$ and $r_{\rm max}$, respectively, for $m_{\rm sh}>10^6M_\odot/h$.
%Being consistent with the two-dimensional plot shown in figure~\ref{fig:contour_Vmax_rmax_1e6}, the $r_{\rm max}$ distribution extends to much lower values of $r_{\rm max}$, while the $V_{\rm max}$ distribution hardly changes.
%In contrast to the CDM case, the rotation curves of the collapsed SIDM subhalos reach a similar maximum velocity at a much smaller radius, reflecting their higher concentration.

%In many cases for the collapsed subhalos, the values of $r_s$ are much smaller than those of the core radius $r_c$. 
%In the regime of $r_s \ll r \ll r_c$, the SIDM density profile goes as $\rho_{\rm sh, SIDM} \propto r^{-2}$ that is iso-thermal and much steeper than the NFW profile.

%\propto \frac{1}{(\sigma_0/m_\chi) (r^{\rm CDM}_s)^{1-n} (\rho^{\rm CDM}_s)^{(3-n)/2}}

%In particular, the core-collapse timescale goes as 
%\begin{equation}
%    t_c\propto \frac{1}{\rho_{\chi}(\sigma/m_{\chi}) v} \propto \frac{1}{\rho_s (\sigma_0/m_{\chi})v^{1-n}} \propto r_s^{n-1} \rho_s^{(n-3)/2} \propto M^{(n-1)/3}c^{(n-7)/2}, \label{eq:cc_scaling}
%\end{equation}


%where $\rho_{\chi}$ is the dark matter density, $\sigma\sim \sigma_0 v^{-n}$ is the SIDM cross section and we used $v\propto \rho_s^{-1/2}$, $M\propto \rho_s r_s^3$, and $c\propto \rho_s^{1/3}$.
